A type reduction theory for systems with replicated components

The Parameterised Model Checking Problem asks whether an implementation Impl(t) satisfies a specification Spec(t) for all instantiations of parameter t. In general, t can determine numerous entities: the number of processes used in a network, the type of data, the capacities of buffers, etc. The main theme of this paper is automation of uniform verification of a subclass of PMCP with the parameter of the first kind, i.e. the number of processes in the network. We use CSP as our formalism. We present a type reduction theory, which, for a given verification problem, establishes a function \phi that maps all (sufficiently large) instantiations T of the parameter to some fixed type T^ and allows us to deduce that if Spec(T^) is refined by \phi(Impl(T)), then (subject to certain assumptions) Spec(T) is refined by Impl(T). The theory can be used in practice by combining it with a suitable abstraction method that produces a t-independent process Abstr that is refined by {\phi}(Impl(T)) for all sufficiently large T. Then, by testing (with a model checker) if the abstract model Abstr refines Spec(T^), we can deduce a positive answer to the original uniform verification problem. The type reduction theory relies on symbolic representation of process behaviour. We develop a symbolic operational semantics for CSP processes that satisfy certain normality requirements, and we provide a set of translation rules that allow us to concretise symbolic transition graphs. Based on this, we prove results that allow us to infer behaviours of a process instantiated with uncollapsed types from known behaviours of the same process instantiated with a reduced type. One of the main advantages of our symbolic operational semantics and the type reduction theory is their generality, which makes them applicable in a wide range of settings.

==> thresholds.tex <==
\subsection{Conditions on processes}\label{section:typereductionpreliminaries}

In this section we start by defining the notion of type symmetry in the
type~$t$; our main theorems will require the implementation process to satisfy
this property.  We then define a property concerning the use of equality
tests; our main theorems will require the specification process to satisfy
this property.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Type symmetry}

In Section~\ref{section:dataindep} we defined the concept of data independence
which, undoubtedly, is a very useful property for studying parameterised
systems
\cite{Creese:1998,Roscoe:1999,Creese:1999a,Lowe:2004,Roscoe:2004}. However, in
practice it turns out to be too strong for the implementations we consider,
since we study parallel compositions of node processes indexed over the
parameter. Such compositions are banned by data independence. This is why we
define a weaker condition, which only requires all behaviours of a given
process to be \emph{symmetric} in the parameter.  A process syntax
satisfies the \textbf{TypeSym} condition if the behaviours of all its
concretisations are invariant under permutations of values of parameter
instantiations. 
%
\begin{defi}\label{def:typesym}\newnot{TypeSym}
A process syntax $Proc(t)$ satisfies the condition \textbf{TypeSym} if
$Proc(T)$ and $Proc(T) \rename{^{\pi(e)} / _e | e \in \Sigma}$ are bisimilar
for every~$T$ and every bijection $\pi: T  \rightarrow T$.  
\end{defi}

Note that the above definition insists that $Proc(t)$ is fully symmetric.  For
example, a system that communicates using a ring topology, where each node~$i$
can send messages only to the node~$(i+1) \bmod N$ (where $N = \#T$) will not
satisfy \textbf{TypeSym}: if $T = \set{0 \upto 4}$ then $Proc(T)$ might have a
trace $\trace{send.1.2}$, but will not have the trace $\trace{send.1.3}$.

Semantic definitions, like the one above, tend to be hard to check
efficiently. So we note here sufficient syntactic conditions for
\textbf{TypeSym}.

\begin{prop}\label{typesymproposition}
A process syntax $Proc(t)$ satisfies the
condition\ \mbox{\textbf{TypeSym}}\ if it uses no 
\begin{enumerate}[(i)]
\item constants of type $t$;

\item operations on type $t$, including polymorphic operations
  (e.g.~tupling or lists); 

\item functions whose domains or co-domains involve type $t$;

\item selections or indexing from sets involving $t$, unless the
  selection or indexing is over the whole of $t$, except this restriction does
  not apply to the alphabets of nodes in a parallel composition indexed
  over~$t$; and  

\item conditional choices on $t$, except for equality and inequality
  tests. 
\end{enumerate}
\end{prop}

%% \begin{remark}\label{remark:tornottindexing}
%% Let
%% $\Extchoice\hspace{-0.68em}\raisebox{-0.7ex}{\rule{0.05em}{3.2ex}}\hspace{0.4em}$
%% be one of $\Extchoice$, $\Intchoice$, $\Parallel$ or $\Interleave$. Then,
%% assumption (iv) of Proposition~\ref{typesymproposition} implies that for every
%% syntax term of the form
%% ``$\Extchoice\hspace{-0.68em}\raisebox{-0.7ex}{\rule{0.05em}{3.2ex}}\hspace{0.4em}\ i
%% \in \mathcal{I}(t)$'', the indexing set definition $\mathcal{I}(t)$ does not
%% contain free variables of type $t$. This means that $\Gamma(\mathcal{I}(T)) =
%% \mathcal{I}(T)$ for every instantiation $T$ of type $t$ and every environment
%% $\Gamma$ in $\mathit{Env}(T)$.
%% \end{remark}

\proof[Proof sketch.] %  (of Proposition~\ref{typesymproposition}).]
Let $CSP_t$ be the set of CSP syntaxes parameterised by~$t$, all of whose free
variables (other that $t$ itself) are of type $t$ and which satisfy the
conditions of the proposition. We use $\rename{\pi}$ to denote
$\rename{^{\pi(e)} / _e | e \in \Sigma}$. Then  
\begin{eqnarray*}
\mathcal{B} & = &
   \left\{ 
     \left( P(T)\rename{\Gamma}, 
          (P(T)\envrename{\pi^{-1}(\Gamma)})\rename{\pi} \right) | 
      P(t) \in CSP_t, \Gamma \in Env(T) \right\}
\end{eqnarray*}
is the required strong bisimulation relation.
%%  on the set of CSP processes whose
%% syntaxes satisfy the conditions of Proposition~\ref{typesymproposition}.
The proof is  a structural induction on $P(t)$. 
\qed
\noindent
In~\cite{moffat:2010}, Moffat proves a very similar result, for a larger
fragment of the machine-readable CSP language, including the underlying
functional language.

The syntactic definition of data independence
(Definition~\ref{def:dataindependence}) comprises a superset of the
requirements of Proposition~\ref{typesymproposition}, so we immediately have
the following result.

\begin{cor}\label{corollary:DIimpliesTypeSym}
Every data independent process satisfies \textbf{TypeSym}. 
\end{cor}

%% The syntactic requirements defined by Proposition~\ref{typesymproposition} are
%% sufficient, but not necessary for $Proc(t)$ to satisfy \textbf{TypeSym}, as
%% the following example illustrates. 

%% \begin{example}
%% Let 
%% \[
%% 	Proc(t) = \If\ c = c \Then \STOP \Else \STOP,
%% \]
%% where $c$ is a constant of type $t$. Then clearly for every $T$, $Proc(T)$ is
%% bisimilar to $\STOP$ . Therefore, $Proc(T)$ is bisimilar to $Proc(T)
%% \rename{\raisebox{0.5ex}{\scriptsize $\pi(e)$} / _e | e \in \Sigma}$ for every
%% $T$ and every bijection $\pi: T  \rightarrow T$. Hence, $Proc(t)$ satisfies
%% the semantic definition of \textbf{TypeSym}. However, it uses constants of
%% type $t$, so it fails the syntactic requirements defined above. 
%% \end{example}


\begin{example}
Consider a system built as the parallel composition of node
processes~$\mathcal{N}_{i}(t)$ for each~$i \in t$:
\begin{eqnarray*}
Nodes(t) & = & \mathop{\Parallel} i \in t \spot [A(i,t)]\ \mathcal{N}_{i}(t) .
\end{eqnarray*}
This process syntax satisfies \textbf{TypeSym} provided:
%
\begin{iteMize}{$\bullet$}
\item
the node process $\mathcal{N}_{i}(t)$ satisfies the conditions of
Proposition~\ref{typesymproposition}, so in particular it treats its
``identity'' parameter~$i$ polymorphically; informally, different nodes need
to be identical up to renaming of the identities;

\item
the alphabet $A(i,t)$ satisfies the conditions of
Proposition~\ref{typesymproposition}, so in particular any selection from~$t$
is over the whole of~$t$; informally, the different alphabets depend only on
the identities~$i$, polymorphically. 
\end{iteMize}
Note, though, that $Nodes(t)$ does not satisfy data independence, since it
contains a replicated operator (parallel composition) that is indexed
over~$t$. 

Further, if we define the context $C_t[.]$ that composes its argument with a
controller process $Ctrl$ and hides some events:
\begin{eqnarray*}
C_t[X] & = & (X \parallel[A] Ctrl) \hide B
\end{eqnarray*}
then $C_t[ Nodes(t) ]$ satisfies \textbf{TypeSym} provided:
\begin{iteMize}{$\bullet$}
\item
the controller process $Ctrl$ satisfies the conditions of
Proposition~\ref{typesymproposition}; informally, it needs to treat different
nodes in the same way;

\item
the sets $A$ and~$B$ satisfy the conditions of
Proposition~\ref{typesymproposition}.
\end{iteMize}
Recall that this is the type of implementation process that we considered in
the Introduction.  In particular, the example from Section~\ref{sec:example}
meets this pattern. 
\end{example}

%% The following example is more concrete than the previous.
%% %
%% \begin{example}\label{tsymexample1}
%% Let
%% \begin{eqns}
%% WORKER = input?data\mathrm{:}Data \then output.(data,f(data)) \then WORKER,
%% \nl
%% WORKERS(t) = \Interleave i \in t \spot WORKER,
%% \nl
%% SERVER(Q_{in},Q_{out}) = \\*
%% \qquad \align
%% 	in?data\mathrm{:}Data \then SERVER(Q_{in}\union \set{data},Q_{out})\\
%% 	\extchoice\\
%% 	\#Q_{in} > 0\ \&\ input?data\mathrm{:}Q_{in} \then
%%           SERVER(Q_{in}\setminus\set{data}, Q_{out})\\
%% 	\extchoice\\
%% 	output?dataAndResult:Data\times Result \then \\
%% 	\qquad SERVER(Q_{in}, Q_{out} \union \set{dataAndResult}) \\
%% 	\extchoice\\
%% 	\#Q_{out} > 0\ \&\ out?dataAndResult\mathrm{:}Q_{out} \then \\
%% 	\qquad SERVER(Q_{in}, Q_{out}\setminus\set{dataAndResult}),
%% 	\endalign \vspace{1ex}
%% \nl
%% SYSTEM(t) = \\*
%% \qquad
%%   (SERVER(\nullset,\nullset) \parallel[\set{|input,output|}] WORKERS(t))
%%      \hide \set{|input,output|} .
%% \end{eqns}
%% Process $SYSTEM(T)$ models a system with a server and $\#T$  workers,
%% where: the server receives packets of data to be processed using the $in$
%% channel and adds then to its input queue $Q_{in}$; the server sends packets of
%% data waiting in the input queue to arbitrary workers using the $input$
%% channel; workers process data and send the result (modelled by $f(data)$) back
%% to the server using the $output$ channel; the server stores arriving results
%% in its output queue $Q_{out}$; and the server sends results waiting in the
%% output queue to the environment using the $out$ channel.
%% %% Process syntax $SYSTEM(t)$ does not satisfy data independence, since it
%% %% contains a replicated operator (interleaving) that is indexed
%% %% over~$t$. However, it does not contain constants of type~$t$, operations on
%% %% type~$t$, functions whose domains or co-domains involve type~$t$,
%% %% selections or indexing from sets involving $t$, or conditional choices
%% %% on~$t$, so by Proposition~\ref{typesymproposition}, $SYSTEM(t)$ satisfies
%% %% \textbf{TypeSym}.
%% \end{example}


\begin{example}
The process 
\(
\Extchoice y\mathrm{:}t \spot c?x\mathrm{:}(t\setminus\set{y})!y 
  \then \STOP
\)
satisfies \textbf{TypeSym}.  However, it does not satisfy the conditions of
Proposition~\ref{typesymproposition}, in particular because $x$ is selected
from a proper subset of~$t$.
\end{example}

The following remark is a direct consequence of the \textbf{TypeSym}
condition.
%
\begin{remark}\label{symtraceremark}\label{symfailureremark}
Suppose that $Proc(t)$ satisfies \textbf{TypeSym}. Then, for all $T$:
%
\begin{iteMize}{$\bullet$}
\item
If $tr \in \tsem{Proc(T)}$ then for all bijections $\pi: T
\rightarrow T$,\, $\pi(tr) \in  \tsem{Proc(T)}$;

\item
If $(tr,X) \in \fsem{Proc(T)}$ then for all bijections $\pi: T
\rightarrow T$,\, $(\pi(tr), \pi(X)) \in  \fsem{Proc(T)}$.
\end{iteMize}
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Equality tests}

The syntactic condition \textbf{PosConjEqT}, formulated by Lazi\'{c}
in~\cite[Chapter 3]{Lazic:1998}, specifies that for a conditional choice with
an equality test on~$t$, the positive branch is a prefix and the negative
branch is simply $\STOP$. In~\cite{Roscoe:1998,Roscoe:1999}, a weaker version
of \textbf{Pos\-Conj\-EqT} is discussed, where no restriction on the process
in the positive branch is in place. Both of these definitions talk about the
condition only in relation to the traces model, but it is easy to extend it to
other models of CSP as the following definition shows.  

\begin{defi}\label{posconjeqt}
Given a CSP model $\mathcal{M}$ we say that a process syntax $Proc(t)$ satisfies \textbf{PosConjEqT$_\mathcal{M}$}\newnot{PosConjEqT} if for every conditional choice on $t$ of the form
\[\If cond \Then P(x_1,\ldots,x_k) \Else Q(x_1,\ldots,x_k)\]
within $Proc(t)$, we have that 
\begin{iteMize}{$\bullet$}
	\item $cond$ is a positive conjunction of equality tests on~$t$ (which gives rise to the name of the condition), and
 	\item $P(v_1,\ldots,v_k) \refinedby_\mathcal{M} Q(v_1,\ldots,v_k)$ for all values $v_1, \ldots, v_k$.
\end{iteMize}
\end{defi}

\noindent For technical reasons, it will be desirable in our work to assume
the opposite condition for specifications: that every positive branch of a
conditional choice is a refinement of the negative branch. This can be viewed
as a reversed version of \textbf{PosConjEqT$_\mathcal{M}$}. Hence, we have the
following definition.

\begin{defi}\label{revposconjeqt}\newnot{RevPosConjEqT}
Given a CSP model $\mathcal{M}$ we say that a process syntax $Proc(t)$
satisfies \textbf{RevPosConjEqT$_\mathcal{M}$} if for every conditional choice
on $t$ of the form 
\[\If cond \Then P(x_1,\ldots,x_k) \Else Q(x_1,\ldots,x_k)\]
within $Proc(t)$, we have that 
\begin{iteMize}{$\bullet$}
	\item $cond$ is a positive conjunction of equality tests on~$t$, and
 	\item $Q(v_1,\ldots,v_k) \refinedby_\mathcal{M} P(v_1,\ldots,v_k)$ for all values $v_1, \ldots v_k$.
\end{iteMize}
\end{defi}
Whenever $\mathcal{M}$ is clear from the context, we will simply
write \textbf{Rev\-Pos\-Conj\-EqT}. 

\begin{example}
The process syntax
\[
Proc(t) =
\align
	in?x\mathrm{:}t?y\mathrm{:}t?z\mathrm{:}t \then \If x = y\ 
	\align
		\Then out.x  \then out.y \then \STOP\\
		\Else out\$z \then (out.y \then \STOP \intchoice \STOP)\\
	\endalign
\endalign
\]
satisfies \textbf{RevPosConjEqT$_\mathrm{F}$}. However, the process syntax
\[
Proc(t) = in?x\mathrm{:}t?y\mathrm{:}t \then \If x = y\ 
\align
	\Then out.x \then \STOP\\
	\Else out.y \then \STOP\\
\endalign
\]
does not satisfy \textbf{RevPosConjEqT$_\mathrm{T}$}, because if $x$ and $y$
are two distinct values, then \mbox{$out.y \then \STOP \not \trefinedby out.x
  \then \STOP$}. 
\end{example}

Most specification processes that one tends to use in practice do not contain
conditionals, so vacuously satisfy both \textbf{PosConjEqT$_\mathcal{M}$} and
\textbf{RevPosConjEqT$_\mathcal{M}$} for all models~$\mathcal{M}$.  Further,
our experience is that many specifications that do contain conditionals
satisfy \textbf{RevPosConjEqT$_\mathcal{M}$}.



